Finding Failures in High-Fidelity Simulation using Adaptive Stress Testing and the Backward Algorithm

Validating the safety of autonomous systems generally requires the use of high-fidelity simulators that adequately capture the variability of real-world scenarios. However, it is generally not feasible to exhaustively search the space of simulation scenarios for failures. Adaptive stress testing (AST) is a method that uses reinforcement learning to find the most likely failure of a system. AST with a deep reinforcement learning solver has been shown to be effective in finding failures across a range of different systems. This approach generally involves running many simulations, which can be very expensive when using a high-fidelity simulator. To improve efficiency, we present a method that first finds failures in a low-fidelity simulator. It then uses the backward algorithm, which trains a deep neural network policy using a single expert demonstration, to adapt the low-fidelity failures to high-fidelity. We have created a series of autonomous vehicle validation case studies that represent some of the ways low-fidelity and high-fidelity simulators can differ, such as time discretization. We demonstrate in a variety of case studies that this new AST approach is able to find failures with significantly fewer high-fidelity simulation steps than are needed when just running AST directly in high-fidelity. As a proof of concept, we also demonstrate AST on NVIDIA's DriveSim simulator, an industry state-of-the-art high-fidelity simulator for finding failures in autonomous vehicles.

==> Images/table_parameters.tex <==
\npdecimalsign{.}
\nprounddigits{1}
\sisetup{round-mode=places,round-precision=2}
\begin{tabular}{@{}lrrr@{}}
\toprule
      Variable & Easy & Medium & Hard \\ \midrule
      {$\beta$} & {\num{1000}} & {\num{0}} & {\num{0}} \\
{$\vect{s}_{0, ped, y}$}      & {$\SI{-4}{\meter} $}  & {$\SI{-6}{\meter}$} & {$\SI{-6}{\meter}$}\\
{$T$}         & {\num{50} steps} & {\num{50} steps} & {\num{100} steps} \\
{$dt$}      & {$\SI{0.1}{\second} $}   & {$\SI{0.1}{\second} $} & {$\SI{0.05}{\second} $} \\
\bottomrule
\end{tabular}
\npnoround

==> Images/table_results.tex <==
\npdecimalsign{.}
\nprounddigits{1}
\sisetup{round-mode=places,round-precision=1}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Algorithm & \shortstack{Steps to\\Failure} & \shortstack{Final\\Reward} & \shortstack{Load Lofi\\Policy?} & \shortstack{Lofi\\Steps} \\\midrule
BA        & NoLoadSteps      & NoLoadReward & No                & LofiSteps              \\
BA        & LoadSteps        & LoadReward   & Yes               & LofiSteps              \\
Hifi      & HifiSteps        & HifiReward   & --                & --                     \\
\bottomrule
\end{tabular}
\npnoround
